Predicting Out-of-Distribution Error with the Projection Norm

We propose a metric -- Projection Norm -- to predict a model's performance on out-of-distribution (OOD) data without access to ground truth labels. Projection Norm first uses model predictions to pseudo-label test samples and then trains a new model on the pseudo-labels. The more the new model's parameters differ from an in-distribution model, the greater the predicted OOD error. Empirically, our approach outperforms existing methods on both image and text classification tasks and across different network architectures. Theoretically, we connect our approach to a bound on the test error for overparameterized linear models. Furthermore, we find that Projection Norm is the only approach that achieves non-trivial detection performance on adversarial examples. Our code is available at https://github.com/yaodongyu/ProjNorm.

==> abstract_previous.tex <==
% abstract v3
% We propose a heuristic for predicting a model's performance on out-of-distribution (OOD) data without  access to ground truth labels. 
% Our method uses pseudolabels of the test samples predicted by the model to retrain a new model. We introduce a notion of distance between the original model and the new model, called {\em Projection Norm}, in the parameter space. Both empirical results and rigorous analysis on linear models suggest this norm is very effective in predicting ODD error-- a larger distance indicates a larger predicted error.  
% Our method, {\em Projection Norm},  first uses model predictions to pseudo-label test samples, then trains a new model on the pseudo-labeleds. The more this model's parameters differ from an in-distribution model, the greater the predicted OOD error. 
% Empirically, our approach outperforms existing methods on both image and text classification tasks, across different network architectures. Theoretically, we connect our approach to a bound on the test error for overparameterized linear models. %and show that linearized network representations accurately predict the error of their nonlinear counterparts. 
% Furthermore, we find that---unlike existing methods---Projection Norm is the only currently proposed measure that achieves non-trivial detection performance on adversarial examples.
%Finally, we bridge the theory and the practice by exactly computing linearized models (neural tangent kernels) on the CIFAR dataset to justify the specific linear model we proposed.

% abstract v2
% In this paper, we propose a method for predicting model performance on out-of-distribution (OOD) data without having access to ground truth labels.
% Our method, ProjectionNorm,  first uses model predictions to pseudolabel test samples, then trains a new model on the pseudo-labeled test set.
% % It then outputs the distance in parameter space to this new model---larger distances indicate a larger predicted error.
% It then outputs the distance from the pre-existing model to this new model in parameter space---larger distances indicate a larger predicted error.
% %Then, ProjNorm compares the difference between two models to estimate the classification error on test samples, where smaller difference implies better model performance.
% Empirically, our approach outperforms existing methods on several image and text classification tasks and across different network architectures.
% Theoretically, we connect our approach to a bound on the test error for overparameterized linear models, and show that linearized network representations accurately predict the error of their nonlinear counterparts. 
% Furthermore, we also find that ProjectionNorm is the only approach that achieves non-trivial performance under adversarial attacks.
% %Finally, we bridge the theory and the practice by exactly computing linearized models (neural tangent kernels) on the CIFAR dataset to justify the specific linear model we proposed.

% abstract v1
% In this paper, we propose Projection Norm, a general method for predicting the out-of-distribution (OOD) test-time performance of a model without having access to ground truth labels of the OOD data.
% During the test time, the Projection Norm algorithm labels the test samples using $f$ and trains a new model $\tilde{f}$ using the pseudo-labeled test set.
% Then, it compares the discrepancy between $f$ and $\tilde{f}$ to estimate how much the training set information helps the particular test samples.
% Empirically, our simple approach better predicts the test time error compared to many existing baselines on standard vision and natural language benchmarks.
% Theoretically, we propose a linear model that naturally motivates the method and provide tight bound on test error.
% Finally, we bridge the theory and the experiment by exactly computing the linearized networks (neural tangent kernels) of vision data to justify the specific linear model we proposed.

